Counterexample-Guided Strategy Improvement for POMDPs Using Recurrent Neural Networks

We study strategy synthesis for partially observable Markov decision processes (POMDPs). The particular problem is to determine strategies that provably adhere to (probabilistic) temporal logic constraints. This problem is computationally intractable and theoretically hard. We propose a novel method that combines techniques from machine learning and formal verification. First, we train a recurrent neural network (RNN) to encode POMDP strategies. The RNN accounts for memory-based decisions without the need to expand the full belief space of a POMDP. Secondly, we restrict the RNN-based strategy to represent a finite-memory strategy and implement it on a specific POMDP. For the resulting finite Markov chain, efficient formal verification techniques provide provable guarantees against temporal logic specifications. If the specification is not satisfied, counterexamples supply diagnostic information. We use this information to improve the strategy by iteratively training the RNN. Numerical experiments show that the proposed method elevates the state of the art in POMDP solving by up to three orders of magnitude in terms of solving times and model sizes.

==> pics/DRNNLayers.tex <==
\def\layersep{2.5cm}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=blue!50];
    \tikzstyle{output neuron}=[neuron, fill=red!25];
    \tikzstyle{hidden neuron}=[neuron, fill=green!25];    
    \tikzstyle{hidden neuron2}=[neuron, fill=green!50];
    \tikzstyle{annot} = [text width=4em, text centered]
    \tikzstyle{annot2} = [text width=8em, text centered];

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:] (I-\name) at (0,-\y cm) {};

%    % Draw the hidden layer nodes
%	\foreach \name / \y in {1,...,3}
%		\path[yshift=-0.25cm]
%			node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};


    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,3}
        \path[yshift=-0.25cm]
            node[hidden neuron2] (H-\name) at (\layersep,-\y cm) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,4}
	    \node[output neuron,pin={[pin edge={->}]right:$a_{\y}$}, right of=H-2](Out-\name) at (\layersep,-\y) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,3}
            \path (I-\source) edge (H-\dest);

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,3}
	    \foreach \dest in {1,...,4}
	        \path (H-\source) edge (Out-\dest);

    % Annotate the layers
    \node[annot2,above of=H-1, node distance=1cm] (hl) {LSTM layer\\$|\ObsSym|/2$ nodes};
%    \node[annot2,left of=hl] (h2) {Hidden layer\\$|\ObsSym|$ nodes};
%    \node[draw,dotted,fit=(H1-1)(H1-3)](Feat){};
    \node[annot2,above of=I-1,node distance=0.8cm] {Input layer \\$|\ObsSym|$ nodes};
    \node[annot,right of=hl] {Output layer};
    \node[draw,dotted,fit=(H-1)(H-3)](LSTM){};
%    \path (Feat) edge [thick] (LSTM);
    \path (LSTM) edge [->, in = 250, out =290,looseness=3,thick] (LSTM);
\end{tikzpicture}
